Flag: a Self-Dual Modality for Non-Commutative Contraction and Duplication in the Category of Coherence Spaces

After reminding what coherences spaces are and how they interpret linear logic, we define a modality "flag" in the category of coherence spaces (or hypercoherences) with two inverse linear (iso)morphisms: "duplication" from (flag A) to ((flag A) < (flag A)) and "contraction" in the opposite direction -- where < is the self dual and non-commutative connective known as "before" in pomset logic and known as "seq(ential)" in the deep inference system (S)BV. In addition, as expected, the coherence space A is a retract of its modal image (flag A). This suggests an intuitive interpretation of (flag A) as "repeatedly A" or as "A at any instant" when "before" is given a temporal interpretation. We hope the semantic construction of flag(A) will help to design proof rules for "flag" and we briefly discuss this at the end of the paper.

==> eptcsdata.tex <==
\providecommand{\firstpage}{157}
\providecommand{\publicationstatus}{U. Dal Lago and V. de Paiva (Eds.) Second Joint International\\ Workshop on Linearity \& Trends in Linear Logic and Applications.\\
EPTCS 353, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.353.8}{10.4204/EPTCS.353.8}}
\pdfoutput=1

